Deep Metric Learning with Chance Constraints

Deep metric learning (DML) aims to minimize empirical expected loss of the pairwise intra-/inter- class proximity violations in the embedding space. We relate DML to feasibility problem of finite chance constraints. We show that minimizer of proxy-based DML satisfies certain chance constraints, and that the worst case generalization performance of the proxy-based methods can be characterized by the radius of the smallest ball around a class proxy to cover the entire domain of the corresponding class samples, suggesting multiple proxies per class helps performance. To provide a scalable algorithm as well as exploiting more proxies, we consider the chance constraints implied by the minimizers of proxy-based DML instances and reformulate DML as finding a feasible point in intersection of such constraints, resulting in a problem to be approximately solved by iterative projections. Simply put, we repeatedly train a regularized proxy-based loss and re-initialize the proxies with the embeddings of the deliberately selected new samples. We applied our method with 4 well-accepted DML losses and show the effectiveness with extensive evaluations on 4 popular DML benchmarks. Code is available at: https://github.com/yetigurbuz/ccp-dml

==> paper/figures/fig_ablation_radius_test.tex <==
% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------

\begin{figure}[!ht]
%\begin{wrapfigure}[14]{r}[-5pt]{0.60\linewidth}
%\vspace{-1.2\intextsep}
	\centering
  \centerline{\includegraphics[width=0.8\linewidth,keepaspectratio]{paper/figures/test_radius.jpg}}

\caption{The geometry of the embedding space\textsuperscript{\protect\hyperlink{figmagnified}{\faSearch}} before, (a), and after, (b), our method (through iterations 1-3), relating how the generalization efforts in training domain transfer to the geometry of test domain on CUB dataset with C2-CCP. We use 2-D TSNE embeddings of the validation data in the visualization, in which we report MAP@R, average covering radius and average inter-class pairwise distances.}
\label{fig:radius_test}
%\end{wrapfigure}
\end{figure}

==> paper/figures/table_all_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

\begin{table*}[!ht]
\centering
\caption{Comparison\textsuperscript{\protect\hyperlink{tabmagnified}{\faInfo}} with the existing methods for the retrieval task on SOP, InShop, CUB, Cars}
\label{tab:all_results}
\resizebox{1.\textwidth}{!}{%
\begin{tabular}{@{}ccc|cc|cc|cc|cc|cc|cc|cc@{}}
\cmidrule(l){2-17}
\multicolumn{1}{l}{}                & \multicolumn{4}{c|}{\textbf{SOP}}                                                                                                                             & \multicolumn{4}{c|}{\textbf{In-shop}}                                                                                                                          & \multicolumn{4}{c|}{\textbf{CUB}}                                                                                                                             & \multicolumn{4}{c}{\textbf{Cars196}}                                                                                                                         \\ \cmidrule(l){2-17} 
                                    & \multicolumn{2}{c|}{\textbf{512D}}                                            & \multicolumn{2}{c|}{\textbf{128D}}                                            & \multicolumn{2}{c|}{\textbf{512D}}                                            & \multicolumn{2}{c|}{\textbf{128D}}                                            & \multicolumn{2}{c|}{\textbf{512D}}                                            & \multicolumn{2}{c|}{\textbf{128D}}                                            & \multicolumn{2}{c|}{\textbf{512D}}                                            & \multicolumn{2}{c}{\textbf{128D}}                                            \\ \cmidrule(l){2-17} 
\textbf{Method}                     & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        & \textbf{P@1}                          & \textbf{MAP@R}                        \\ \midrule
\multicolumn{1}{c|}{C1}             & 68.84                                 & 40.25                                 & 64.96                                 & 36.54                                 & 80.12                                 & 50.15                                 & 76.08                                 & 46.51                                 & 63.67                                 & 23.08                                 & 56.21                                 & 19.06                                 & 77.75                                 & 23.50                                 & 64.17                                 & 16.13                                 \\
\multicolumn{1}{c|}{C1-XBM-L}       & 78.68                                 & 51.82                                 & 75.37                                 & 47.39                                 & 88.39                                 & 58.64                                 & \textbf{85.75}                        & 55.37                                 & 65.40                                 & 24.87                                 & 57.57                                 & 19.84                                 & 83.68                                 & 27.93                                 & \textbf{72.13}                        & 18.83                                 \\
\multicolumn{1}{c|}{C1-CCP-L}      & {\color[HTML]{FE0000} \textbf{79.53}} & {\color[HTML]{FE0000} \textbf{52.73}} & {\color[HTML]{FE0000} \textbf{76.24}} & {\color[HTML]{FE0000} \textbf{48.07}} & \textbf{88.52}                        & \textbf{59.67}                        & 85.50                                 & \textbf{55.56}                        & \textbf{68.11}                        & \textbf{27.11}                        & \textbf{59.56}                        & \textbf{21.27}                        & \textbf{83.76}                        & \textbf{28.32}                        & 72.05                                 & \textbf{18.96}                        \\ \midrule
\multicolumn{1}{c|}{C2}             & 74.87                                 & 46.94                                 & 71.15                                 & 42.66                                 & 86.32                                 & 59.42                                 & 83.04                                 & 55.13                                 & 67.49                                 & 26.47                                 & 59.73                                 & 21.01                                 & 81.04                                 & 24.73                                 & 69.17                                 & 17.22                                 \\
\multicolumn{1}{c|}{C2-XBM-L}       & 76.66                                 & 49.04                                 & 73.47                                 & 45.15                                 & 87.66                                 & 60.64                                 & 84.58                                 & 56.75                                 & 68.62                                 & 26.83                                 & 60.18                                 & 21.41                                 & 82.40                                 & 25.99                                 & 70.01                                 & 18.01                                 \\
\multicolumn{1}{c|}{C2-CCP-L}      & \textbf{78.95}                        & \textbf{52.19}                        & \textbf{75.92}                        & \textbf{48.18}                        & \textbf{88.52}                        & \textbf{61.07}                        & \textbf{86.11}                        & \textbf{57.24}                        & {\color[HTML]{FE0000} \textbf{69.73}} & {\color[HTML]{FE0000} \textbf{28.02}} & {\color[HTML]{FE0000} \textbf{62.39}} & {\color[HTML]{FE0000} \textbf{22.67}} & \textbf{82.89}                        & \textbf{26.27}                        & \textbf{72.16}                        & \textbf{18.52}                        \\ \midrule
\multicolumn{1}{c|}{MS}             & 72.74                                 & 44.10                                 & 68.96                                 & 40.18                                 & 88.37                                 & 60.65                                 & 85.39                                 & 56.61                                 & 64.65                                 & 24.15                                 & 57.24                                 & 19.64                                 & 80.88                                 & 26.23                                 & 69.27                                 & 18.25                                 \\
\multicolumn{1}{c|}{MS-CCP-L}      & \textbf{78.96}                        & \textbf{51.85}                        & \textbf{75.80}                        & \textbf{47.97}                        & {\color[HTML]{FE0000} \textbf{90.24}} & \textbf{63.59}                        & {\color[HTML]{FE0000} \textbf{87.10}} & {\color[HTML]{FE0000} \textbf{59.15}} & \textbf{68.84}                        & \textbf{27.44}                        & \textbf{61.10}                        & \textbf{22.40}                        & {\color[HTML]{FE0000} \textbf{86.26}} & {\color[HTML]{FE0000} \textbf{29.14}} & \textbf{74.97}                        & {\color[HTML]{FE0000} \textbf{19.85}} \\ \midrule
\multicolumn{1}{c|}{Triplet}        & 75.40                                 & 47.03                                 & 70.41                                 & 41.03                                 & 86.71                                 & 60.60                                 & 82.58                                 & 55.25                                 & 64.01                                 & 23.43                                 & 55.51                                 & 18.51                                 & 78.44                                 & 23.11                                 & 64.57                                 & 15.68                                 \\
\multicolumn{1}{c|}{Triplet-CCP-L} & \textbf{77.09}                        & \textbf{49.33}                        & \textbf{72.21}                        & \textbf{43.11}                        & \textbf{89.44}                        & {\color[HTML]{FE0000} \textbf{64.28}} & \textbf{86.00}                        & \textbf{59.04}                        & \textbf{65.36}                        & \textbf{24.53}                        & \textbf{56.65}                        & \textbf{19.31}                        & \textbf{81.84}                        & \textbf{25.21}                        & \textbf{68.75}                        & \textbf{17.43}                        \\ \midrule
\multicolumn{1}{c|}{ProxyAnchor}    & 77.10                                 & 49.01                                 & 73.86                                 & 44.89                                 & 88.08                                 & 58.09                                 & 85.87                                 & 54.95                                 & 68.43                                 & 26.53                                 & 60.61                                 & 21.48                                 & 85.29                                 & 27.73                                 & {\color[HTML]{FE0000} \textbf{75.79}} & 19.56                                 \\
\multicolumn{1}{c|}{ProxyNCA++}     & 76.07                                 & 48.20                                 & 72.89                                 & 44.44                                 & 87.33                                 & 57.48                                 & 84.79                                 & 54.42                                 & 65.48                                 & 24.85                                 & 58.49                                 & 20.96                                 & 82.87                                 & 26.34                                 & 72.45                                 & 19.32                                 \\
\multicolumn{1}{c|}{SoftTriple-S/L}   & 78.48                                 & 50.77                                 & 74.66                                 & 45.75                                 & 88.37                                 & 59.56                                 & 85.71                                 & 55.68                                 & 66.12                                 & 26.02                                 & 57.94                                 & 19.86                                 & 84.90                                 & 27.80                                 & 73.16                                 & 19.18                                 \\ \bottomrule
\end{tabular}%
}
\end{table*}
